Superfast amplification and superfast nonlinear saturation of perturbations as the mechanism of turbulence

Ruelle predicted that the maximal amplification of perturbations in homogeneous isotropic turbulence is exponential $e^{\sigma \sqrt{Re} t}$ (where $\sigma \sqrt{Re}$ is the maximal Liapunov exponent). In our earlier works, we predicted that the maximal amplification of perturbations in fully developed turbulence is faster than exponential $e^{\sigma \sqrt{Re} \sqrt{t} +\sigma_1 t}$. That is, we predicted superfast initial amplification of perturbations. Built upon our earlier numerical verification of our prediction, here we conduct a large numerical verification with resolution up to $2048^3$ and Reynolds number up to $6210$. Our direct numerical simulation here confirms our analytical prediction. Our numerical simulation also demonstrates that such superfast amplification of perturbations leads to superfast nonlinear saturation. We conclude that such superfast amplification and superfast nonlinear saturation of ever existing perturbations serve as the mechanism for the generation, development and persistence of fully developed turbulence.

==> bibtitle.tex <==

\bibitem{RT71} D. Ruelle and F. Takens, On the nature of turbulence, Comm. Math. Phys. {\bf 20}, 167 (1971).

\bibitem{BJPV05} T. Bohr, M. H. Jensen, G. Paladin, and A. Vulpiani, {\it
Dynamical Systems Approach to Turbulence} (Cambridge University Press, 2005).

\bibitem{KK01} G. Kawahara, S. Kida, Periodic motion embedded in plane Couette turbulence: regeneration cycle and burst, J. Fluid Mech. {\bf 449}, 291 (2001).

\bibitem{Vis07} D. Viswanath, Recurrent motions within plane Couette turbulence, J. Fluid Mech.
{\bf 580}, 339 (2007).

\bibitem{GHC08} J. F. Gibson, J. Halcrow, and P. Cvitanovi\'c, Visualizing the geometry of state space in plane Couette flow, J. Fluid Mech. {\bf 611}, 107 (2008).

\bibitem{VK11} L. van Veen and G. Kawahara, Homoclinic tangle on the edge of shear turbulence,
Phys. Rev. Lett. {\bf 107}, 114501 (2011).

\bibitem{KUV12} G. Kawahara, M. Uhlmann, and L. van Veen, The significance of simple invariant solutions in turbulent flows, Ann. Rev. Fluid Mech. {\bf 44}, 203 (2012).

\bibitem{KE12} T. Kreilos and B. Eckhardt, Periodic orbits near onset of chaos in plane Couette flow, Chaos {\bf 22}, 047505 (2012).

\bibitem{LK15} D. Lucas, R. Kerswell, Recurrent flow analysis in spatiotemporally chaotic 2-dimensional Kolmogorov flow, Phys. Fluids {\bf 27}, 045106 (2015).

\bibitem{Rue79} D. Ruelle, Microscopic fluctuations and turbulence, Phys. Lett. {\bf 72A}, 81 (1979).

\bibitem{CJVP93} A. Crisanti, M. H. Jensen, A. Vulpiani, and G. Paladin, Intermittency and predictability in turbulence, Phys. Rev. Lett. {\bf 70}, 166 (1993).

\bibitem{ABCPV96} E. Aurell, G. Boffetta, A. Crisanti, G. Paladin, and A. Vulpiani, Growth of noninfinitesimal perturbations in turbulence, Phys. Rev. Lett. {\bf 77}, 1262 (1996).

\bibitem{ABCPV97} E. Aurell, G. Boffetta, A. Crisanti, G. Paladin, and A. Vulpiani, Predictability in the large: an extension of the concept of Lyapunov exponent, J. Phys. A {\bf 30}, 1 (1997).

\bibitem{BCFV02} G. Boffetta, M. Cencini, M. Falcioni, and A. Vulpiani, Predictability: a way to characterize complexity, Phys. Rep. {\bf 356}, 367 (2002).

\bibitem{MB17} G. Boffetta and S. Musacchio, Chaos and predictability of homogeneous-isotropic turbulence, Phys. Rev. Lett. {\bf 119}, 054102 (2017).

\bibitem{BH18} A. Berera and R. Ho, Chaotic properties of a turbulent isotropic fluid, Phys. Rev. Lett. {\bf 120}, 024101 (2018).

\bibitem{Li14} Y. Li, The distinction of turbulence from chaos --- rough dependence on initial data, Electronic Journal of Differential Equations {\bf 2014}, 104 (2014).

\bibitem{Li17} Y. Li, Rough dependence upon initial data exemplified by explicit solutions and the effect of viscosity, Nonlinearity {\bf 30} 1097 (2017).

\bibitem{Li18} Y. Li, Linear hydrodynamic stability, Notices of the AMS {\bf 65}, 1255 (2018).

\bibitem{Inc15} H. Inci, On the regularity of the solution map of the incompressible Euler equation, Dynamics of Partial Differential Equations {\bf 12}, 97 (2015).

\bibitem{IL18} H. Inci, Y. Li, Nowhere-differentiability of the solution map of 2D Euler equations on bounded spatial domain,  arXiv:1805.06507, http://faculty.missouri.edu/~liyan/2DEuler.pdf (2018).

\bibitem{FL18} Z. Feng and Y. Li, Short term unpredictability of high Reynolds number turbulence — rough dependence on initial data, arXiv:1702.02993,  http://faculty.missouri.edu/~liyan/Rough-Num.pdf (2018).

\bibitem{Yof12} S. R. Yoffe, Investigation of the transfer and dissipation of energy in isotropic turbulence, Ph.D. Thesis, University of Edinburg (2012), arXiv: 1306.3408.

\bibitem{Mac97} L. Machiels, Predictability of small-scale motion in isotropic turbulence, Phys. Rev. Lett. {\bf 79}, 3411 (1997).

\bibitem{KI06} Y. Kaneda and T. Ishihara, High-resolution direct numerical simulation of turbulence, J. of Turbulence {\bf 7}, N20 (2006).

\bibitem{LM15} M. F. Linkmann and A. Morozov, Sudden relaminarization and lifetimes in forced isotropic turbulence, Phys. Rev. Lett. {\bf 115}, 134502 (2015).


